KRED: Knowledge-Aware Document Representation for News Recommendations

News articles usually contain knowledge entities such as celebrities or organizations. Important entities in articles carry key messages and help to understand the content in a more direct way. An industrial news recommender system contains various key applications, such as personalized recommendation, item-to-item recommendation, news category classification, news popularity prediction and local news detection. We find that incorporating knowledge entities for better document understanding benefits these applications consistently. However, existing document understanding models either represent news articles without considering knowledge entities (e.g., BERT) or rely on a specific type of text encoding model (e.g., DKN) so that the generalization ability and efficiency is compromised. In this paper, we propose KRED, which is a fast and effective model to enhance arbitrary document representation with a knowledge graph. KRED first enriches entities' embeddings by attentively aggregating information from their neighborhood in the knowledge graph. Then a context embedding layer is applied to annotate the dynamic context of different entities such as frequency, category and position. Finally, an information distillation layer aggregates the entity embeddings under the guidance of the original document representation and transforms the document vector into a new one. We advocate to optimize the model with a multi-task framework, so that different news recommendation applications can be united and useful information can be shared across different tasks. Experiments on a real-world Microsoft News dataset demonstrate that KRED greatly benefits a variety of news recommendation applications.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> preliminary.tex <==
\section{preliminaries}
%In this section, we introduce some background information including document vectors, knowledge graphs and news recommendation related tasks.
\subsection{Document Representation}
\label{sec:dv}
Precise document representation is the key to the success of news recommendations. There are quite a few document representation methods in literature, such as bag of words, LDA \cite{Blei:2003:LDA:944919.944937}, denoising autoencoder \cite{Okura:2017:ENR:3097983.3098108}, DSSM \cite{Huang:2013:LDS:2541176.2505665}, Kim-CNN \cite{DBLP:conf/emnlp/Kim14}, HAN \cite{yang2016hierarchical} and BERT \cite{DBLP:conf/naacl/DevlinCLT19}. To stay concise, we discuss three of them which stand for different categories of NLU models.
\subsubsection{LDA}
Latent Dirichlet allocation (LDA) \cite{Blei:2003:LDA:944919.944937} is a generative statistical model which can discover the abstract "topics`` of a document. It assumes that each document is a mixture of a set of topics and each word's presence is attributable to one of these topics. LDA is an unsupervised learning model and is not a neural model. Given a document, LDA can associate it to a topic vector $\mathbf{v}_d = \langle s_1, s_2, ..., s_n \rangle$, where $s_j \ (j \in [1,n])$ means the probability of topic j occurring in the document, and $n$ indicates the number of topics.
\subsubsection{DSSM}
Deep Structured Semantic Model (DSSM) \cite{Huang:2013:LDS:2541176.2505665} is a deep neural network modeling technique for representing raw text into a continuous latent space and modeling semantic similarity between text strings. It is a supervised learning model with the label being users' responses. It has been successfully applied in many web applications such as web search ranking and ads selection. Given a document, DSSM performs several non-linear projections and finally transforms it into a latent vector $\mathbf{v}_d \in \mathbb{R}^n$ in a low-dimensional semantic feature space.
\subsubsection{BERT}
Pre-training has proven effective in improving language models. BERT \cite{DBLP:conf/naacl/DevlinCLT19}, which stands for Bidirectional Encoder Representations from Transformers, presents a deep bidirectional pre-training model for language representation and advances state-of-the-art methods for a suite of NLU tasks. We adopt the \textsl{feature-based} strategy to apply representations from BERT, namely to consume the latent vector $\mathbf{v}_d \in \mathbb{R}^n$ as input features for downstream tasks without fine-tuning BERT layers.
\subsection{Knowledge Graph}\label{sec:kg}
A knowledge graph contains enriched and structured side information and has shown to be helpful for recommendation systems. Here we formulate a knowledge graph as a collection of entity-relation-entity triples: $\mathcal{G}=\{(h,r,t)|h,t\in \mathcal{E}, r\in \mathcal{R}\}$, where $\mathcal{E}$ and $\mathcal{R}$ represent the set of entities and relations respectively, $(h,r,t)$ represents that there is a relation $r$ from $h$ to $t$. We assume that entities which appear in one news article can be linked to the corresponding entities in the knowledge graph.

In order to utilize information from the knowledge graph, we resort to a knowledge graph embedding technique which can learn a low-dimensional representation vector for entities and relations. In practice, any kind of graph embedding method can be used here, while for simplicity purpose we introduce TransE \cite{Bordes:2013:TEM:2999792.2999923} in this paper. TransE learns embedding vectors $\textbf{e} \in \mathbb{R}^d$ for each entity and relationship, so that $\textbf{e}_h + \textbf{e}_r \approx \textbf{e}_t$ when $(h,r,t)$ holds. The learning process minimizes the following margin-based ranking criterion over the training triplets:
\begin{equation}
     \mathcal{L} = \sum_{(h,r,t)\in\Delta}\sum_{(h',r,t')\in\Delta'} max(0, f_d(\textbf{e}_h+\textbf{e}_r, \textbf{e}_t) + \gamma - f_d(\textbf{e}_{h'}+\textbf{e}_r, \textbf{e}_{t'}))
\end{equation}
where $\gamma>0$ is a margin hyperparameter, $f_d$ is a dissimilarity measure such as the $L_1$ and the $L_2$-norm, and $\Delta, \Delta'$ are the set of correct triplets and incorrect triplets.
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.85\textwidth,trim={0 0cm 0 0},clip]{figures/doc_embedding.pdf}%
    \caption{An overview of the proposed \emph{KRED} model.}
     %\vspace{-0.1in}
    \label{fig:overall_KDV}
\end{figure*}
\subsection{News Recommendation Applications}
Different from most existing works which study only item recommendations, we study four applications in news recommendations.
\subsubsection{Item Recommendation} 
This is the most widely studied application. Given a user $i$, let $\{d_1^i, d_2^i,...,d_t^i\}$ denotes his/her click history, where $d_j^i$ denotes the $j$-th news article clicked by the user. We want to recommend personalized new articles to him/her in the future based on the click history.
\subsubsection{News Popularity Prediction} New popularity prediction application is important in several aspects. First, in the candidate retrieval layer of an industrial recommender system, usually there are various recall methods including personalized and non-personalized methods. Retrieving popular items is one of the most commonly used non-personalized methods. Second, precise forecasting of news popularity can help editors select high-quality articles, especially in the headline channel. Third, for personalized ranking models, the popularity level of an item is an important feature. We take this task as a multi-class classification problem.
\subsubsection{Local News Detection} In this application, we want to predict whether a news article reports an event that happens in a local context that would not be an interest of another locality. This is a binary classification problem.
\subsubsection{News Category Classification} This application predicts the category label that a news article belongs to. We have 15 top-level categories in the news corpus. Thus this is a multi-class classification problem.
